Provable Constrained Stochastic Convex Optimization with XOR-Projected Gradient Descent

Provably solving stochastic convex optimization problems with constraints is essential for various problems in science, business, and statistics. Recently proposed XOR-Stochastic Gradient Descent (XOR-SGD) provides a convergence rate guarantee solving the constraints-free version of the problem by leveraging XOR-Sampling. However, the task becomes more difficult when additional equality and inequality constraints are needed to be satisfied. Here we propose XOR-PGD, a novel algorithm based on Projected Gradient Descent (PGD) coupled with the XOR sampler, which is guaranteed to solve the constrained stochastic convex optimization problem still in linear convergence rate by choosing proper step size. We show on both synthetic stochastic inventory management and real-world road network design problems that the rate of constraints satisfaction of the solutions optimized by XOR-PGD is $10\%$ more than the competing approaches in a very large searching space. The improved XOR-PGD algorithm is demonstrated to be more accurate and efficient than both XOR-SGD and SGD coupled with MCMC based samplers. It is also shown to be more scalable with respect to the number of samples and processor cores via experiments with large dimensions.

==> tex/constrained_case.tex <==
\section{Extension to the Constrained Case}\label{app:constrain_XOR-SGD}

In this part, we are able to quantify the convergence speed of algorithm \ref{alg:constrain_XOR-SGD} to the optimum if the problem only contains equality constraints. 
%
In this case, we solve the problem $\min_x\max_{\lambda} F(x,\lambda)$ with the following augmented Lagrangian function
\begin{align}\label{eq:minmax_linear}
    F(x,\lambda)= \mathbb{E}_{\theta}[f(x,\theta)]+\lambda^T(Ax+b)+\frac{\beta}{2}||Ax+b||^2
\end{align}
where $A\in \mathbb{R}^{m\times n}$ is a full-rank matrix and $b$ is a vector, indicating the linear equality constraints. $\beta$ is a hyperparameter, which does not change in the optimization process. 
%
See Corollary \ref{Co:primal_dual}. Our proof is extended from \cite{ouyang2013stochastic} and \cite{alghunaim2020linear}.  


For the analysis below, we consider an alternating direction algorithm, and assume that
$M$ is large enough for the algorithm to find the optimal value $x_{k+1}$ in the $k-$th iteration.  in algorithm \ref{alg:constrain_XOR-SGD}
%
This version of the alternating optimization algorithm becomes the commonly known primal-dual gradient method. 
%We show the primal-dual XOR-SGD in algorithm \ref{alg:primal-dual_XOR-SGD}, where $x$ and $\lambda_i,\mu_j$ are optimized together iteratively. To our best knowledge, 
We can prove the convergence rate of this algorithm when only equality constraints are added. Specifically, 
Let $\sigma_i(A)$ be its $i$-th largest singular value, and let $\sigma_{\max}(A)=\sigma_1(A)$ and $\sigma_{\min}(A)=\sigma_{\min\{m,n\}}(A)$ be the largest and the smallest non-zero singular values of $A$, respectively. We also use $f(x)$ to represent $\mathbb{E}_{\theta}[f(x,\theta)]$ for short.
In practice we update $x$ in the $k-$th iteration using an approximated augmented Lagrangian:
\begin{align}\label{eq:approx-x}
    L_{k}(x,\lambda)=&f(x_k)+f'(x_k,\theta_{k+1})x+\lambda^T(Ax+b)\notag\\
    &+\frac{\beta}{2}||Ax+b||^2+\frac{||x-x_k||^2}{2\eta_{k+1}}
\end{align}
where we replace $f(x)$ with a first-order approximation of $f(x,\theta_{k+1})$, and add a $l_2-$norm prox-function scaled by a time-varying step size $\eta_{k+1}$. Then we have the following theorem:

\begin{Th}\label{Th:primal-dual}
In the setting of Algorithm \ref{alg:constrain_XOR-SGD} to solve problem in equation \ref{eq:minmax_linear} with only linear equality constraints, if we update $x$ according to equation \ref{eq:approx-x}, then Algorithm exhibits a rate of $O(\frac{1}{\sqrt{K}})$ of convergence in terms of the objective value. Specifically, denote $x^*$ the optimal value of $x$, let $\max_x\mathbb{E}[||\nabla f(x,\theta)||^2]\leq M^2$, $D_{X}=sup_{x_a,x_b\in \mathcal{X}}||x_a-x_b||$, and learning rate $\eta_k=\frac{D_{X}}{M\sqrt{2k}}$ for all $k\geq 1$.
Define $M(K)=\frac{\sqrt{2}\rho\kappa D_{X}M}{\sqrt{K}}+\frac{\tau^2}{2\beta K}$, where $\rho\kappa$ is the constant approximation of gradients. Then for $obj=\mathbb{E}_{\theta}[f(\overline{x_K},\theta)]$, $OPT=\mathbb{E}_{\theta}[f(x^*,\theta)]$ and $\forall \tau>0$, we have
\begin{align}\label{eq:primal-dual}
    \mathbb{E}_x[obj-OPT+\tau||A\overline{x_K}+b||^2]\leq M(K)
\end{align}
\end{Th}
The proof of Theorem \ref{Th:primal-dual} is based on two lemmas. We will start with the following simple lemma,
which is a very useful result by implementing Bregman divergence as a prox-function in proximal methods.
\begin{Lm}\label{Lm:1}
Let $f(x):\mathcal{X}\rightarrow \mathbb{R}$ be a convex differentiable function with gradient $g$. Let scalar $s\geq 0$. For any vector $u$ and $v$, denote their Bregman divergence as $D(u,v)=\omega(u)-\omega(v)-\langle\nabla\omega(v),u-v\rangle$ for a differentiable function $\omega(\cdot)$. If $u\in\mathcal{X}$, and 
\begin{align}
    x^*=\text{argmin}_{x\in\mathcal{X}} f(x)+sD(x,u),
\end{align}
then, 
\begin{align*}
    \langle g(x^*), x^*-x\rangle\leq s[D(x,u)-D(x,x^*)-D(x^*,u)].
\end{align*}
\end{Lm}
\begin{proof} (Lemma \ref{Lm:1})~~
The optimality condition implies
\begin{align*}
    \langle g(x^*)+s\nabla D(x^*,u), x^*-x\rangle \geq 0, ~~~\forall x\in\mathcal{X}
\end{align*}
which is equal to
\begin{align*}
     \langle g(x^*), x^*-x\rangle\leq& s\langle \nabla D(x^*,u), x-x^*\rangle\\
     =& s\langle \nabla \omega(x^*)-\nabla\omega(u), x-x^*\rangle\\
     =& s[D(x,u)-D(x,x^*)-D(x^*,u)].
\end{align*}
This completes the proof.
\end{proof}
Utilizing the Lemma \ref{Lm:1}, we are able to obtain an upper bound of the variation of the Lagrangian function and its first order approximation based on each iteration points, which is shown in Lemma \ref{Lm:2}.
\begin{Lm}\label{Lm:2}
Let $w=(x,\lambda)$, $F(w)=(A^T\lambda, Ax+b)$ and $\delta_{k}=f'(x_{k-1},\theta_k)-f'(x_{k-1})$, then for $\forall w\in\mathcal{W}$ and $k\geq 0$ we have
\begin{align*}
    &f(x_k)-f(x)+(w_{k+1}-w)^TF(w_{k+1})\leq \rho\kappa \langle \delta_{k+1}, x-x_k \rangle\\
    &+\frac{\eta_{k+1}\rho\kappa||f'(x_k,\theta_{k+1})||^2}{2}+\frac{\rho\kappa(||x_k-x||^2-||x_{k+1}-x||^2)}{2\eta_{k+1}} \\
    &+\frac{1}{2\beta}(||\lambda-\lambda_k||^2-||\lambda-\lambda_{k+1}||^2)
\end{align*}
\end{Lm}

\begin{proof} (Lemma \ref{Lm:2})~~
Due to the convexity of $f$ we have
\begin{align*}
    f(x_k)-f(x)&\leq \langle f'(x_k),x_k-x \rangle\leq \rho\kappa(\langle f'(x_k,\theta_{k+1}),x_{k+1}-x \rangle\\ 
    &+ \langle \delta_{k+1},x-x_k \rangle + \langle f'(x_k, \theta_{k+1}),x_k-x_{k+1} \rangle)
\end{align*}
Applying Lemma \ref{Lm:1} to equation \ref{eq:approx-x} and taking $D(u,v)=\frac{1}{2}||v-u||^2$, we have
\begin{align*}
    &\langle f'(x_k,\theta_{k+1}) + A^T[\beta(Ax_{k+1}+b)-\lambda_{k}],x_{k+1}-x \rangle\\
    &\leq \frac{\rho\kappa}{2\eta_{k+1}}(||x_k-x||^2-||x_{k+1}-x||^2-||x_{k}-x_{k+1}||^2)
\end{align*}
Combining the above two inequalities we have
\begin{align*}
    &f(x_k)-f(x)+\langle x_{k+1}-x,A^T\lambda_{k+1}  \rangle\\
    \leq& \rho\kappa\langle f'(x_k,\theta_{k+1}),x_{k+1}-x \rangle + \rho\kappa\langle \delta_{k+1},x-x_k \rangle\\
    &+ \frac{1}{2\beta}||\lambda_k-\lambda_{k+1}||^2+ \rho\kappa\langle f'(x_k, \theta_{k+1}),x_k-x_{k+1} \rangle\\
    &+ \langle x_{k+1}-x, A^T[\beta(Ax_{k+1}+b)-\lambda_{k}] \rangle\\
    \leq& \frac{\rho\kappa}{2\eta_{k+1}}(||x_k-x||^2-||x_{k+1}-x||^2-||x_{k}-x_{k+1}||^2)\\
    &+ \rho\kappa\langle \delta_{k+1},x-x_k \rangle + \rho\kappa\langle f'(x_k, \theta_{k+1}),x_k-x_{k+1} \rangle\\
    &+ \frac{1}{2\beta}||\lambda_k-\lambda_{k+1}||^2
\end{align*}
For the last term, we have
\begin{align*}
    &\langle f'(x_k, \theta_{k+1}),x_k-x_{k+1} \rangle\\
    \leq& \frac{\eta_{k+1}||f'(x_k,\theta_{k+1})||^2}{2} + \frac{||x_k-x_{k+1}||^2}{2\eta_{k+1}}
\end{align*}
where the last step is due to Young's inequality. Therefore, we have
\begin{align*}
    &f(x_k)-f(x)+\langle x_{k+1}-x,A^T\lambda_{k+1}  \rangle\\
    \leq& \frac{\rho\kappa}{2\eta_{k+1}}(||x_k-x||^2-||x_{k+1}-x||^2)+ \frac{1}{2\beta}||\lambda_k-\lambda_{k+1}||^2\\
    &+\frac{\eta_{k+1}\rho\kappa||f'(x_k,\theta_{k+1})||^2}{2} + \rho\kappa\langle \delta_{k+1},x-x_k \rangle 
\end{align*}
For the optimization of $\lambda$, we have
\begin{align*}
    &\langle \lambda_{k+1}-\lambda, Ax_{k+1}+b \rangle=\frac{1}{\beta}\langle \lambda_{k+1}-\lambda, \lambda_{k}-\lambda_{k+1} \rangle\\
    =&\frac{1}{2\beta}(||\lambda-\lambda_k||^2-||\lambda-\lambda_{k+1}||^2-||\lambda_k-\lambda_{k+1}||^2)
\end{align*}
Taking the summation of the inequalities above, we obtain the desired result.
\end{proof}

Then, we are ready to prove Theorem \ref{Th:primal-dual}.
\begin{proof}~~(Theorem \ref{Th:primal-dual})~~
Since $f$ is convex and $F(w)$ is monotonic. we have
\begin{align*}
    &f(\overline{x_{K}})-f(x)+(\overline{w_K}-w)^TF(\overline{w_K})\\
    \leq& \frac{1}{K}\sum_{k=1}^{K}[f(x_{k-1})-f(x)+(w_k-w)^TF(w_k)]\\
    =&\frac{1}{K}\sum_{k=0}^{K-1}[f(x_{k})-f(x)+(w_{k+1}-w)^TF(w_{k+1})]
\end{align*}
Applying Lemma \ref{Lm:2} at the optimal solution $x=x^*$, we can derive that
\begin{align*}
    &f(\overline{x_{K}})-f(x^*)+(\overline{x_{K}}-x^*)^T(A^T\overline{\lambda_K})+(\overline{\lambda_K}-\lambda)^T(A\overline{x_{K}}+b)\\
    \leq& \frac{\rho\kappa}{K}\sum_{k=0}^{K-1}[ \frac{\eta_{k+1}||f'(x_k,\theta_{k+1})||^2}{2}
    +\frac{||x_k-x||^2-||x_{k+1}-x||^2}{2\eta_{k+1}}\\
    &+\langle \delta_{k+1}, x^*-x_k \rangle ] + \frac{1}{K}(\frac{\beta}{2}||Ax^*+b||^2+\frac{1}{2\beta}||\lambda-\lambda_0||^2)\\
    \leq& \frac{\rho\kappa}{K}\sum_{k=0}^{K-1}[ \frac{\eta_{k+1}||f'(x_k,\theta_{k+1})||^2}{2}+ \langle \delta_{k+1}, x^*-x_k \rangle ]\\
    &+\frac{1}{K}(\frac{\rho\kappa D_X^2}{2\eta_K}+\frac{1}{2\beta}||\lambda-\lambda_0||^2)
\end{align*}
The above inequality holds for all $\lambda\in\mathbb{R}^m$, hence also holds for the ball $\mathcal{B}_0=\{\lambda:||\lambda||\leq \tau\}$. Combing with the fact that the optimal solution must also be feasible, we have 
\begin{align*}
    &\max_{\lambda\in\mathcal{B}_0}\{f(\overline{x_{K}})-f(x^*)+(\overline{x_{K}}-x^*)^T(A^T\overline{\lambda_K})\\
    &\qquad+(\overline{\lambda_K}-\lambda)^T(A\overline{x_{K}}+b)\}\\
    =&\max_{\lambda\in\mathcal{B}_0}\{f(\overline{x_{K}})-f(x^*)+ \overline{\lambda_K}^T(Ax^*+b)-\lambda^T(A\overline{x_K}+b)\}\\
    =&\max_{\lambda\in\mathcal{B}_0}\{f(\overline{x_{K}})-f(x^*)-\lambda^T(A\overline{x_K}+b) \}\\
    =&f(\overline{x_{K}})-f(x^*)+\tau||A\overline{x_K}+b||^2
\end{align*}
Taking the expectation over $x$, we have
\begin{align*}
    &\mathbb{E}[f(\overline{x_{K}})-f(x^*)+\tau||A\overline{x_K}+b||^2]\\
    \leq& \mathbb{E}[\frac{\rho\kappa}{K}\sum_{k=0}^{K-1}( \frac{\eta_{k+1}||f'(x_k,\theta_{k+1})||^2}{2}+\langle \delta_{k+1}, x^*-x_k \rangle)\\
    &+\frac{D_X^2}{2K\eta_K}] + \mathbb{E}[\max_{\lambda\in\mathcal{B}_0}\{\frac{1}{2\beta K}||\lambda-\lambda_0||^2\}]\\
    \leq& \frac{\rho\kappa}{K}(\frac{M^2}{2}\sum_{k=1}^K \eta_{k}+\frac{D_X^2}{2\eta_K})+ \frac{\tau^2}{2\beta K}\\ &+\frac{\rho\kappa}{K}\sum_{k=1}^K \mathbb{E}[\langle \delta_{k+1}, x^*-x_k \rangle]\\
    \leq& \frac{\sqrt{2}\rho\kappa D_{X}M}{\sqrt{K}}+\frac{\tau^2}{2\beta K}
\end{align*}
In the last step, we use the fact that $x_k$ is independent of $\theta_{k+1}$, hence the summation of expectation terms is zero. This completes the proof. 
\end{proof}

% \begin{Th}\label{Th:promal_dual}
% In the setting of Algorithm \ref{alg:constrain_XOR-SGD} to solve problem in equation \ref{eq:minmax_linear} with only linear equality constraints, if we choose $t<\frac{1}{\beta}$ and $\eta\leq\frac{\alpha}{\sigma_{\max}^2}$, and let $\tilde{x}_k=\mathbb{E}[x_k-x^*]$ and $\tilde{\lambda}_k=\mathbb{E}[\lambda_k-\lambda^*]$, then algorithm \ref{alg:constrain_XOR-SGD} converges linearly to the optimal saddle-point $x^*, \lambda^*$, namely, it holds that
% \begin{align}\label{eq:main_eq_cr}
%     c_x||\tilde{x_k}||^2+c_{\lambda}||\tilde{\lambda}_k||^2\leq\gamma(c_x||\tilde{x}_{k-1}||^2+c_{\lambda}||\tilde{\lambda}_{k-1}||^2)
% \end{align}
% where $c_{\lambda}=\frac{t}{\eta}>0$, $c_{x}=1-t\eta\sigma_{\max}^2>0$, and 
% \begin{align*}
%     \gamma=\max\{1-\frac{t\alpha(1-t\beta)}{\rho^2\kappa^2}, 1-t\eta\sigma_{min}^2\}<1.
% \end{align*}

% \end{Th}

% \begin{proof} (Theorem \ref{Th:promal_dual})~~
% Subtracting $x^*$ and $\lambda^*$ from both sides of the updating formula in algorithm \ref{alg:constrain_XOR-SGD} and using the optimality condition, we get the coupled error recursion \xyx{is this true?? In the inner loop of algorithm \ref{alg:constrain_XOR-SGD}, $x$ is not updated with $\lambda$ information.}
% \begin{align*}
%     \tilde{x}_k&=\tilde{x}_{k-1}\\
%     &-t(\mathbb{E}[\nabla \mathbb{E}_{\theta}[f(x_k,\theta)]]-\nabla\mathbb{E}_{\theta}[f(x^*,\theta)]]+A^T\tilde{\lambda}_{k-1})\\
%     \tilde{\lambda}_{k}&=\tilde{\lambda}_{k-1}+\eta A\tilde{x}_k
% \end{align*}
% Squaring both sides, we can get
% \begin{align*}
%     ||\tilde{x}_k||^2&=||\tilde{x}_{k-1}-t(\mathbb{E}[\nabla \mathbb{E}_{\theta}[f(x_k,\theta)]]-\nabla\mathbb{E}_{\theta}[f(x^*,\theta)]]||^2\\
%     &-2t\tilde{\lambda}_{k-1}^TA(\mathbb{E}[\nabla \mathbb{E}_{\theta}[f(x_k,\theta)]]-\nabla\mathbb{E}_{\theta}[f(x^*,\theta)]])\\
%     &+t^2||A^T\tilde{\lambda}_{k-1}||^2
% \end{align*}
% \begin{align*}
%     &||\tilde{\lambda}_{k}||^2=||\tilde{\lambda}_{k-1}||^2+\eta^2||A\tilde{x}_k||^2+2\eta\tilde{\lambda}_{k-1}A\tilde{x}_k\\
%     &=||\tilde{\lambda}_{k-1}||^2+\eta^2||A\tilde{x}_k||^2-2t\eta||A^T\tilde{\lambda}_{k-1}||^2\\
%     &+2\eta\tilde{\lambda}_{k-1}A(\tilde{x}_{k-1}-t(\mathbb{E}[\nabla \mathbb{E}_{\theta}[f(x_k,\theta)]]-\nabla\mathbb{E}_{\theta}[f(x^*,\theta)]]))
% \end{align*}
% Using the bound $||A\tilde{x}_k||^2\leq\sigma_{\max}^2||\tilde{x}_k||^2$ and denoting $c_{\lambda}=\frac{t}{\eta}$ and $c_{x}=1-t\eta\sigma_{\max}^2$, we have 
% \begin{align*}
%     &c_x||\tilde{\lambda}_{k}||^2+c_{\lambda}||\tilde{\lambda}_{k-1}||^2\\
%     \leq & ||\tilde{x}_{k-1}-t(\mathbb{E}[\nabla \mathbb{E}_{\theta}[f(x_k,\theta)]]-\nabla\mathbb{E}_{\theta}[f(x^*,\theta)]]||^2\\
%     + & c_{\lambda}||\tilde{\lambda}_{k-1}||^2-t^2||A^T\tilde{\lambda}_{k-1}||^2
% \end{align*}
% Then, since also $||A^T\tilde{\lambda}_{k-1}||^2\geq\sigma_{min}^2||\tilde{\lambda}_{k-1}||^2$, we can further get
% \begin{align*}
%     &c_x||\tilde{\lambda}_{k}||^2+c_{\lambda}||\tilde{\lambda}_{k-1}||^2\\
%     \leq & ||\tilde{x}_{k-1}-t(\mathbb{E}[\nabla \mathbb{E}_{\theta}[f(x_k,\theta)]]-\nabla\mathbb{E}_{\theta}[f(x^*,\theta)]]||^2\\
%     + & (1-t\eta\sigma_{min}^2)c_{\lambda}||\tilde{\lambda}_{k-1}||^2
% \end{align*}
% Since $\mathbb{E}_{\theta}[f(x_k,\theta)]$ is $\beta$-smooth \xyx{no $x_k$, correct?}, it holds that
% \begin{align*}
%     &||\nabla \mathbb{E}_{\theta}[f(x_{k-1},\theta)]]-\nabla\mathbb{E}_{\theta}[f(x^*,\theta)]]||^2\\
%     \leq & \beta\tilde{x}_{k-1}^T(\nabla \mathbb{E}_{\theta}[f(x_{k-1},\theta)]]-\nabla\mathbb{E}_{\theta}[f(x^*,\theta)]])
% \end{align*}
% Thus
% \begin{align*}
%     &||\tilde{x}_{k-1}-t(\mathbb{E}[\nabla \mathbb{E}_{\theta}[f(x_k,\theta)]]-\nabla\mathbb{E}_{\theta}[f(x^*,\theta)]]||^2\\
%     \leq&(1-\frac{t\alpha(2-t\beta)}{\rho^2\kappa^2})||\tilde{x}_{k-1}||^2
% \end{align*}
% where $t<2/\beta$. This follows directly by expanding the square and considering the $\rho\kappa$ bound from XOR-Sampling.\xyx{why?? why suddenly there comes $\alpha$?} Let $\gamma_1=1-\frac{t\alpha(1-t\beta)}{\rho^2\kappa^2}$, and $c_{x}=1-t\eta\sigma_{\max}^2$, it holds that 
% \begin{align*}
%     &(1-\frac{t\alpha(2-t\beta)}{\rho^2\kappa^2})||\tilde{x}_{k-1}||^2\\
%     &=\gamma_1||\tilde{x}_{k-1}||^2-\frac{t\alpha}{\rho^2\kappa^2}||\tilde{x}_{k-1}||^2\\
%     &\leq \gamma_1c_x||\tilde{x}_{k-1}||^2-\frac{t(\alpha-\eta\sigma_{max}^2\gamma_1)}{\rho^2\kappa^2}||\tilde{x}_{k-1}||^2\\
%     &\leq\gamma_1c_x||\tilde{x}_{k-1}||^2
% \end{align*}
% where the last step we used the fact that the second term is non-positive under the conditions $t<\frac{1}{\beta}$ and $\eta\leq\frac{\alpha}{\sigma_{\max}^2}$. 
% \xyx{where's the reasoning for $\tilt{\lambda}$?} 
% Therefore, we conclude that equation \ref{eq:main_eq_cr} holds by using the results above. Note that $c_x>0$ and $0<1-t\eta\sigma_{min}^2<1$ if $t\eta<\frac{1}{\sigma_{\max}^2}$. This condition is satisfied under the conditions in the theorem because under the condition we have
% \begin{align*}
%     t\eta< \frac{\alpha}{\beta\sigma_{\max}^2}\leq\frac{1}{\sigma_{\max}^2}
% \end{align*}
% where the last inequality holds because $\alpha\leq\beta$. This completes the proof.

% \end{proof}


\subsection{Proof of Corollary 1}
% \subsection{Proof of Corollary \ref{Co:primal_dual}}
Corollary \ref{Co:primal_dual} can be directly obtained based on Theorem \ref{Th:primal-dual}.
% \begin{proof} (Corollary \ref{Co:primal_dual})~~
From Theorem \ref{Th:primal-dual}, we can see $M(k)$ is $O(\frac{1}{\sqrt{k}})$. Therefore, we can directly see that algorithm \ref{alg:constrain_XOR-SGD} has $O(\frac{1}{\sqrt{K}})$ convergence rate towards the optimal value where $K$ is the total number of iterations.
% Because $R_k=c_x||\tilde{x}_k||^2+c_{\lambda}||\tilde{\lambda}_{k}||^2$, we have both $||\tilde{x}_k||^2\leq \frac{R_k}{c_x}$ and $||\tilde{\lambda}_k||^2\leq\frac{R_k}{c_{\lambda}}$. Since from Theorem \ref{Th:promal_dual} we have $R_{k+1}\leq CR_k$ where $0<C<1$, indicating that $R_k$ approaches zero. Therefore, both $||\tilde{x}_k||^2$ and $||\tilde{\lambda}_k||^2$ are also approaching zero. Then, after $k\geq\log(\frac{R_0}{\epsilon\min\{c_x,c_{\lambda}\}}-C)$ iterations, we have $k\log C\leq \log\frac{\epsilon\min\{c_x,c_{\lambda}\}}{R_0}$, which leads to $R_k\leq C^kR_0\leq\epsilon\min\{c_x,c_{\lambda}\}$. Therefore, $||\tilde{x}_k||^2\leq\epsilon$ and $||\tilde{\lambda}_k||^2\leq\epsilon$. This completes the proof.
% \end{proof}
We leave the proof to future work for convex inequality constraints. However, we showed experimentally in several real-world problems that XOR-SGD algorithm outperforms other methods when solving stochastic optimization problems dealing with convex inequality constraints.


==> tex/related.tex <==
XOR-SGD was motivated by \textit{Sample Average Approximation} (SAA)  \cite{kleywegt2002sample,Verweij2003SAA}, which is widely used to solve stochastic optimization problems. 
%
On learning probabilistic graphical models, \textit{the Marginal Maximum-a-posterior (MMAP) problem} \cite{Xue2016MarginalMAP,LiuI13VariationalMMAP,Radu14AndOrMMAP,Maua2012AnytimeMAP,Marinescu2015AOBB,domke2013learning} is related and can be formulated as (albeit non-convex) stochastic optimization problems. 
%
\textit{Convergence analysis of gradient descent} has been studied for both convex and non-convex functions \cite{wang2013variance,dubey2016variance,agarwal2017finding,lee2015distributed,allen2018make,ruder2016overview,jin2017accelerated,ge2015escaping}. Recently several algorithms \cite{duchi2011adaptive,hinton2012neural,kingma2014adam,duchi2018minimax,allen2017katyusha,allen2018natasha} were proposed to accelerate the convergence rate of SGD. 
%
They require an unbiased estimation of either the gradient or the momentum. Our XOR-SGD was derived without this assumption. 
%
However, as future work, we expect to further accelerate XOR-SGD following this line of work by estimating higher order moments with guarantees. 
%Since these terms also have constant bounds, we could further extend our results to these algorithms.
%
\textit{Probabilistic inference via hashing and randomization} is proposed for both sampling \cite{ermon2013embed,ivrii2015computing}, counting \cite{Gomes2006NearUniformSampling,ding2019towards}, and marginal inference  problems \cite{Ermon13Wish,kuck2019adaptive,Chakraborty2014DistributionAwareSA,Chakraborty2015WeightedCounting,belle2015hashing} with constant approximation guarantees. %We further extend this property to guarantee the bound of the solution of an optimization algorithm.
%
\textit{Inventory management} is a classic problem for supply chain management in operational research  \cite{ziukov2016literature} where SAA is often used \cite{shapiro2007tutorial}, nonetheless with no formal guarantees. 
%
Previously a few approaches have been proposed for \textit{network design} \cite{sheldon2012maximizing,WuXSG17XORSampling}. We consider optimizing the commuting time, which is a more challenging objective and to our knowledge, no prior work derives algorithms with guarantees. 


